Noise-Free Score Distillation

Score Distillation Sampling (SDS) has emerged as the de facto approach for text-to-content generation in non-image domains. In this paper, we reexamine the SDS process and introduce a straightforward interpretation that demystifies the necessity for large Classifier-Free Guidance (CFG) scales, rooted in the distillation of an undesired noise term. Building upon our interpretation, we propose a novel Noise-Free Score Distillation (NFSD) process, which requires minimal modifications to the original SDS framework. Through this streamlined design, we achieve more effective distillation of pre-trained text-to-image diffusion models while using a nominal CFG scale. This strategic choice allows us to prevent the over-smoothing of results, ensuring that the generated data is both realistic and complies with the desired prompt. To demonstrate the efficacy of NFSD, we provide qualitative examples that compare NFSD and SDS, as well as several other methods.

==> figures/single_view.tex <==
\iffalse
\begin{figure}
    \centering
    \setlength{\tabcolsep}{1pt}
    % {\scriptsize
    \begin{tabular}{c C{0.14\linewidth} C{0.14\linewidth} C{0.14\linewidth} C{0.14\linewidth} C{0.14\linewidth} C{0.14\linewidth} C{0.14\linewidth}}
        \raisebox{15pt}{\rotatebox{90}{ SDS $100$}} &
        \includegraphics[width=\linewidth]{images/single/unsolid/dragon_mosaic/sds.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/dragon_two_heads/sds.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/orangutan/sds.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/hedgehog/sds.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/sds/peacock.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/sds/armadillo.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/sds/cookies.jpg}         
        \\
        %
        \raisebox{15pt}{\rotatebox{90}{ NFSD $7.5$}} &
        \includegraphics[width=\linewidth]{images/single/unsolid/dragon_mosaic/nfsd.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/dragon_two_heads/nfsd.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/orangutan/nfsd.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/hedgehog/nfsd.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/nfsd/peacock.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/nfsd/armadillo.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/nfsd/cookies.jpg}  

        \\
        %
        &
        ``A metal lying Buddha'' &
        ``A cake made of ice'' &
        ``A photo of subset, winter, river'' &
        ``A white dog sleeping'' &
        ``A fire with smoke''&
        ``A photo of subset, winter, river'' &
        ``A fire with smoke''
        % ``Panda snowboarding'' &
        % ``A white cat sleeping
        \\
    \end{tabular}
    % }
    \caption{Comparison of Single-view latent-Nerf via SDS (second row) and NFSD (first row).}
    \label{fig:single-view}
\end{figure} 
\fi

\begin{figure}
    \centering
    \setlength{\tabcolsep}{1pt}
    % {\scriptsize
    \begin{tabular}{ C{0.14\linewidth}  C{0.14\linewidth} C{0.02\linewidth} C{0.14\linewidth} C{0.14\linewidth} C{0.02\linewidth} C{0.14\linewidth} C{0.14\linewidth}}
        SDS & NFSD & &
        SDS & NFSD & &
        SDS & NFSD  
        \\     
        \includegraphics[width=\linewidth]{images/single/unsolid/dragon_mosaic/sds.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/dragon_mosaic/nfsd.jpg} &
         &
        \includegraphics[width=\linewidth]{images/single/unsolid/dragon_two_heads/sds.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/dragon_two_heads/nfsd.jpg} &
        &
        \includegraphics[width=\linewidth]{images/single/unsolid/hedgehog/sds.jpg} &
        \includegraphics[width=\linewidth]{images/single/unsolid/hedgehog/nfsd.jpg} 
        %\vspace{-0.2\linewidth}  
        %\\
        %
       % &
        %\multicolumn{2}{c}{``Decorative mosaic of the mythological Chinese dragon''} & &
        %\multicolumn{2}{c}{``A two headed fire dragon with small wings''} & &
        %\multicolumn{2}{c}{``A huge Hedgehog''} 
        \\
        \includegraphics[width=\linewidth]{images/single/solid/sds/peacock.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/nfsd/peacock.jpg} &
         &
        \includegraphics[width=\linewidth]{images/single/solid/sds/armadillo.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/nfsd/armadillo.jpg} &
        &
        \includegraphics[width=\linewidth]{images/single/solid/sds/cookies.jpg} &
        \includegraphics[width=\linewidth]{images/single/solid/nfsd/cookies.jpg} 
		%\vspace{-0.2\linewidth}        
        %\\
        %
       % &
        %\multicolumn{2}{c}{``A a peacock with wings spread''} & &
        %\multicolumn{2}{c}{``Nine banded armadillo'} & &
        %\multicolumn{2}{c}{``A plate piled high with chocolate chip cookies''} 
        \\        
        
       % ``A white dog sleeping'' &
       % ``A fire with smoke''&
       % ``A photo of subset, winter, river'' &
       % ``A fire with smoke''
        % ``Panda snowboarding'' &
        % ``A white cat sleeping
        %\\
    \end{tabular}
    % }
    \caption{Comparison of Narrow-view latent-Nerf via SDS  and NFSD. NFSD exhibits greater detail and clarity when compared to SDS100. Supplementary files contain the prompts for reference.}
    \label{fig:single-view}
\end{figure} 
